Pessimistic Minimax Value Iteration: Provably Efficient Equilibrium Learning from Offline Datasets

We study episodic two-player zero-sum Markov games (MGs) in the offline setting, where the goal is to find an approximate Nash equilibrium (NE) policy pair based on a dataset collected a priori. When the dataset does not have uniform coverage over all policy pairs, finding an approximate NE involves challenges in three aspects: (i) distributional shift between the behavior policy and the optimal policy, (ii) function approximation to handle large state space, and (iii) minimax optimization for equilibrium solving. We propose a pessimism-based algorithm, dubbed as pessimistic minimax value iteration (PMVI), which overcomes the distributional shift by constructing pessimistic estimates of the value functions for both players and outputs a policy pair by solving NEs based on the two value functions. Furthermore, we establish a data-dependent upper bound on the suboptimality which recovers a sublinear rate without the assumption on uniform coverage of the dataset. We also prove an information-theoretical lower bound, which suggests that the data-dependent term in the upper bound is intrinsic. Our theoretical results also highlight a notion of "relative uncertainty", which characterizes the necessary and sufficient condition for achieving sample efficiency in offline MGs. To the best of our knowledge, we provide the first nearly minimax optimal result for offline MGs with function approximation.

==> illustrating_example.tex <==
% Illustrating example
\tank{I restate the example in the previous note here.}
\begin{theorem}
  Consider a class of bandit tabular games with deterministic reward and their datasets
  $$ \mathcal{G} = \{(\mathcal{M},\mathcal{D})|\{(a_i,b_j)|\pi^*(a_i)\nu^*(b_j)\neq 0)\}\subset\mathcal{D},\pi^*\otimes\nu^*\text{being the NE of} \ \mathcal{M}\}  $$ 
  For any algorithm,  there exists $ (\mathcal{M},\mathcal{D}))\in \mathcal{G} $ such that the output of the algorithm $ (\hat{\pi},\hat{\nu}) $bsatisfying 
  $$ \sub(\hat{\pi},\hat{\nu}) \geq 1. $$      
\end{theorem}
\begin{proof}
  Consider the following two games. The payoff matrices of games $ \mathcal{M}_1,\mathcal{M}_2 $  are
  \begin{equation*}
    R_1 = \left(
    \begin{array}{ccc}
      0.5 & -1 & 0  \\
      1 & \textcolor{red}{0} & 1  \\
      0 & -1 & 0  \\
    \end{array}\right), R_2 = \left(
      \begin{array}{ccc}
        0 & 0 & -1  \\
        1 & 0 & -1  \\
        1 & 1 & \textcolor{red}{0}  \\
      \end{array}\right).
  \end{equation*}
  The entries with red color are the NE of the games.We consider the dataset
  $ \mathcal{D} = \{(a_2,b_2),(a_3,b_3)\}. $
  Then $ (\mathcal{M}_1,\mathcal{D}),(\mathcal{M}_2,\mathcal{D})\in\mathcal{G}. $ But when players take actions that are in $ \mathcal{D} $,  the reward of these two games are the same. As a result, the algorithm cannot distinguish these two games. Suppose that the output policies are 
  $ \pi(a_i) = p_i,\nu(b_j) = q_j,$ we can easily compute the suboptimality.
  $$ \sub_{\mathcal{M}_1}(\hat{\pi},\hat{\nu}) = 2-p_2-q_2,\qquad \sub_{\mathcal{M}_2}(\hat{\pi},\hat{\nu}) = p_1+q_1+p_2+q_2.$$
  Therefore, $ \sub_{\mathcal{M}_1}(\hat{\pi},\hat{\nu}) + \sub_{\mathcal{M}_2}(\hat{\pi},\hat{\nu})\geq2 $, which implies $ \sub_{\mathcal{M}_1}(\hat{\pi},\hat{\nu})\geq 1$ or $ \sub_{\mathcal{M}_2}(\hat{\pi},\hat{\nu})\geq 1$ .          
\end{proof}
The intuition behind the preceding theorem is that supposed the algorithm play game $ \mathcal{M}_1 $, however, with limited information, the payoff matrix in the eye of the algorithm becomes 
\begin{equation*}
  R = \left(
  \begin{array}{ccc}
    * & * & *  \\
    * & 0 & *  \\
    * & * & 0  \\
  \end{array}\right).
\end{equation*}
 $ '*' $ means that the algorithm has no any information on these actions. Thus we may change the value of the $ * $ entries to find $ \mathcal{M}_2 $ such that the algorithm cannot play well in both of the games. The real problem is that unlike the case of MDP\cite{jin2020pessimism}, it's insufficient for the algorithm to determine the NE only with the NE information. However, an important observation enable us to make an assumption that is weaker than the uniform coverage assumption. That is, if the actions $G =  \{(a_1,b_2),(a_2,b_2),(a_2,b_1),(a_2,b_3),(a_3,b_2)\} $ are covered by the dataset, the payoff matrix in the eye of the algorithm becomes 
 \begin{equation*}
  R = \left(
  \begin{array}{ccc}
    * & \mathbf{-1} & *  \\
    \mathbf{1} & \textcolor{red}{0} & \mathbf{1}  \\
    * & \mathbf{-1} & *  \\
  \end{array}\right).
\end{equation*}
  In this case, however we change the $ '*' $ entries, we will not change the game's NE. Intuitively, for sufficiently smart algorithms, they can identify the NE with information from $ G $ . Indeed, that's the case. We will prove it in Section \label{sec:illustration}. The set $ G $ also motivates us to consider a new concept, the Related Uncertainty(RU).

==> section2.tex <==
\section{Suboptimality Decomposition}
    In the following three section, we mainly focus on two-player zero-sum MG. All the game mentioned in these section is assumed to be this kind of game unless otherwise specified. In this section, we try to give an answer to the problem that what cause the suboptimality of an algorithm by giving a decomposition of it. 
    \par $\quad$We know that the value function and Q-function of any policy pair should satisfy  equation (\ref{eq:bellmam_eq}), but in practice, usually, algorithms can only approximate these two functions, which will no longer satisfy this equation. This error can be measured by the following quantity. It turns out that the following Bellman error play an important role in the cause of suboptimality.
  \#\iota^{(i)}_{h}(s,a,b) = \mathbb{B}_h\widehat{V}_{h+1}^{(i)}(s,a,b)-\qfunhat_h(s,a,b)\label{def:iota}\#
  where $V^{(i)}_h$ is the approximated value function of the game from the perspective of player $i$ at step $h$.
  \begin{theorem}[Decompostion of Suboptimality]\label{theorem:sub_decomp}
    Let $(\widehat{\pi},\nuhat) = \{(\widehat{\pi}_h,\nuhat_h)\}_{h = 1}^H $be a product policy. The approximated value function of player $i$ $\valuefunhat_h^{(i)}(x)$ and Q-function $ \qfunhat_h^{(i)}(\cdot,\cdot,\cdot)$satisfy 
    \$
    \valuefunhat_h^{(i)}(x) = \langle\widehat{Q}_h^{(i)}(x,\cdot,\cdot),\widehat{\pi}_h(\cdot|x) \otimes \nuhat_h(\cdot|x)\rangle_{\mathcal{A}_1 \times \mathcal{A}_2} 
    \$ 
    where $\cdot \otimes \cdot$ is the tensor product of two vectors and $\langle\cdot,\cdot\rangle_{\mathcal{A}_1\times\mathcal{A}_2}$ is the inner product of the two vectors. For any pairs $(\pihat,\nuhat)$ and $x \in \mathcal{S} $, we have  
    \begin{align}\label{eq:subopt_decomp}  
      &V_1^*(x)-V_1^{\pihat,\nuhat}(x) \\
      &= 
  - \underbrace{\sum_{h = 1}^H \expect_{\pihat,\vhat}\left[\iota^{(1)}_{h}(s_h,a_h,b_h)|s_1=x\right]}_\mathlarger{\text{Spurious Correlation for P1}} \\
  & +\underbrace{\sum_{h = 1}^H \expect_{\pi^*,\vhat}\left[\iota^{(1)}_{h}(s_h,a_h,b_h)|s_1=x\right]}_\mathlarger{\text{Related Uncertainty for P1}} \notag\\
  &+\underbrace{\sum_{h = 1}^H \expect_{\pi^*,\vhat}\left[\langle\qfunhat^{(1)}_h(s_h,\cdot,\cdot),(\pi_h^* (\cdot|s_h)-\pihat_h(\cdot|s_h))\otimes\vhat_h(\cdot|s_h)\rangle_{\mathcal{A}_1 \times\mathcal{A}_2 }|s_1=x\right]}_\mathlarger{\text{Optimization Error for P1}} \notag \\
  &+\underbrace{\sum_{h = 1}^H \expect_{\pi^*,\vhat}\left[\langle Q_h^*(s_h,\cdot,\cdot),\pi_h^* (\cdot|s_h)\otimes(\nu_h^*(\cdot|s_h)-\vhat_h(\cdot|s_h))\rangle_{\mathcal{A}_1 \times \mathcal{A}_2 }|s_1=x\right]}_\mathlarger{\text{Optimization Error for P1}}
  \end{align}
  where expectation $\expect_{\pi^*,\nu}$ is taken respect to the trajectory induced by $(\pi^*,\nu)$ in the underlying MG. Similar equation holds for $V_1^{\pihat,\nuhat}(x)-V_1^*(x)$. See Appendix \ref{pf:decomp} for the other equation.
  \end{theorem}
  \begin{proof}[Proof of Theorem \ref{theorem:sub_decomp}]
    See Appendix \ref{pf:decomp} for detailed proof.
  \end{proof}
  Here we choose to use a different version of decomposition rather than directly decompose $V^{\brt(\nuhat),\nuhat}_1(x) - V^{\pihat,\brt(\pihat)}_1(x)$ since our goal is to give an upper bound to the absolute error of value function and we want to achieve the goal with less information. See section \ref{se:LMG} for further explanation. In the case of MDP, one only need to maximize the reward. Let player 2 be a null player we obtain the decomposition in the case of MDP \citep{jin2020pessimism}
  \begin{corollary}
    Supposed $(\mcm,\mbp,\mathcal{A},r)$ is a MDP. $\pi^*$ is the best policy of the MDP. Let $\pihat$ be a policy, such that the approximated value function $\valuefunhat(x)$ and Q-function $ \qfunhat(\cdot,\cdot)$ satisfy $\valuefunhat_h(x) = \langle\qfunhat_h(x,\cdot),\pihat_h\rangle_{\mathcal{A}}$. Let $\iota_{h}(s_h,a_h) = \bellman\valuefunhat_h(s_h,a_h)-\qfunhat_h(s_h,a_h)$ We have 
    \begin{align*}
      V_1^*(x)-V_1^{\pihat}(x) &= - \sum_{h = 1}^H \expect_{\pihat}\left[\iota_{h}(s_h,a_h)|s_1=x\right] + \sum_{h = 1}^H \expect_{\pi^*}\left[\iota_{h}(s_h,a_h)|s_1=x\right] \\
      &+\sum_{h = 1}^H \expect_{\pi^*}\left[\langle\qfunhat_h(s_h,\cdot),\pi_h^* (\cdot|s_h)-\pihat_h(\cdot|s_h)\rangle_{\mathcal{A}}|s_1=x\right]
    \end{align*}
  \end{corollary}


==> section3.tex <==

\section{Suboptimality of the Pessimistic Algorithm}
In this section, first, we give a pessimistic algorithm and estimation of its suboptimality for general Markov Game. Then, we consider a specific kind of Markov Game, the Linear Markov Game, where we additionally assume the linearity of the transition kernel and reward function.

\subsection{General Version}
  In value iteration algorithm, one need to construct an approximated Bellman operator $\bellmanhat $ base on the dataset. $\mathcal{D}$. $(\bellmanhat\valuefunhat_{h+1})(\cdot,\cdot,\cdot): \mathcal{S}\times\mathcal{A}_1\times\mathcal{A}_2 \rightarrow \mathbb{R}$ give an estimation of of the real Q-function $Q_h(\cdot,\cdot,\cdot)$. Then, one use it to calculate the value function iteratively and use the estimated function to make judgement. However, the traditional algorithm ignores the 'uncertainty' of the approximated Bellman operator, which may cause considerable amount of spurious correlation, contributing to the suboptimality of the algorithm. Thus, we introduce the following notion to characterize this 'uncertainty'.

  \begin{definition}[$p$-uncertainty quantifer] \label{def:p_uncerty}
     $\Gamma_h(s,a,b)$ is a $p$-uncertainty quantifier with respect to $P_{\mathbb{D}} $ if the event 
        \#
        &\mathcal{E}=\{|\bellmanhat \widehat{V}_{h+1}^{(i)}(s,a,b)-\mathbb{B}_h\widehat{V}_{h+1}^{(i)}(s,a,b)|\leqslant \Gamma_h(s,a,b), \notag\\
        & \qquad \forall (s,a,b) \in \mathcal{S} \times  \mathcal{A}_1 \times \mathcal{A}_2,h\in [H],i = 1,2 \} \label{eq:p_uncerty}
        \#
        happens with probability $\mathbb{P}_{\mathcal{D}}(\mathcal{E})\geqslant 1-p$.
  \end{definition}
        
        $\quad$The notion of $p$-uncertainty enable us to measure the uncertainty of constructed Bellman operator. Analogy to to UCB algorithm, we can use $\Gamma_h(\cdot,\cdot,\cdot)$ to give a pessimistic estimation of the Q-function, which gives the following algorithm. 

  \begin{algorithm}[h] 
    \caption{Nash-PEVI for Two-player General Markov Game}
    \begin{algorithmic}[1]
    \STATE Input Dataset $\mathcal{D} = \{(s_h^{\tau},a_h^{\tau},b_h^{\tau},r_h^{\tau})\}_{h=1,\tau = 1}^{H,K}$
    \STATE Initialize $\valuefunhat^{(1)}_{H+1},\valuefunhat^{(2)}_{H+1}$ as zero functions.
    \STATE \textbf{For} step $h = H ,H-1, \ldots ,1$ \textbf{do:}
    \STATE \hspace{0.15in} Construct $(\bellmanhat\valuefunhat_{h+1}^{(i)})(\cdot,\cdot,\cdot),\Gamma_h(\cdot,\cdot,\cdot)$ based on the $\mathcal{D}$ .
    \STATE  \hspace{0.15in} Set $\qfunhat_h^{(1)}(\cdot,\cdot,\cdot) \leftarrow  \mathrm{\Pi}_h\left((\bellmanhat\valuefunhat_{h+1}^{(1)})(\cdot,\cdot,\cdot) - \Gamma_h(\cdot,\cdot,\cdot)\right)$.
    \STATE  \hspace{0.15in}  Set $\qfunhat_h^{(2)}(\cdot,\cdot,\cdot) \leftarrow  \mathrm{\Pi}_h\left((\bellmanhat\valuefunhat_{h+1}^{(2)})(\cdot,\cdot,\cdot)+ \Gamma_h(\cdot,\cdot,\cdot)\right)$.
    \STATE  \hspace{0.15in} Set $(\pihat_h,\vhat_h) \leftarrow \text{Find\_NE} \left(\qfunhat_h^{(1)}(\cdot,\cdot,\cdot),\qfunhat_h^{(2)}(\cdot,\cdot,\cdot) \right)$
    \STATE  \hspace{0.15in} Set $\valuefunhat^{(1)}_h(s) \leftarrow \langle\qfunhat_h^{(1)}(s,\cdot,\cdot),\pihat_h(\cdot|s)\otimes \vhat_h(\cdot|s)\rangle_{\mathcal{A}_1 \times \mathcal{A}_2 }$
    \STATE  \hspace{0.15in} Set $\valuefunhat^{(2)}_h(s) \leftarrow \langle\qfunhat_h^{(2)}(s,\cdot,\cdot),\pihat_h(\cdot|s)\otimes \vhat_h(\cdot|s)\rangle_{\mathcal{A}_1 \times \mathcal{A}_2}$
    \STATE  \textbf{End for}
    \STATE   Output Pess  $(\mathcal{D}) = \{(\pihat_h,\vhat_h)\}_{h=1}^H$.

    \end{algorithmic}\label{ALGO:PEVI-UCB_General}
  \end{algorithm}
  $\quad$ In Algorithm \ref{ALGO:PEVI-UCB_General}, we choose to let both of the players make pessimistic estimation of the Q-function since we want to give an upper bound to the absolute error $\abso{V_1^*(x)-V_1^{\pihat,\nuhat}(x)}$, that is, we need to bound the error of both sides. In the online setting \citep[section  4]{xie2020learning}, one only need to maximize the reward of one side, so doing pessimism in one side and using one approximated Q-function to evaluate the NE are enough. 
  
  The following theorem characterizes the suboptimality of Algorithm \ref{ALGO:PEVI-UCB_General}.
    \begin{theorem} \label{theorem:general_gap_upperb}
      Suppose $\{\Gamma_h\}_{h=1}^H$ in Algorithm \ref{ALGO:PEVI-UCB_General} is a $p$-uncertainty quantifier defined in (\ref{def:p_uncerty}). Under $\mathcal{E}$ defined by equation(\ref{eq:p_uncerty}), which happens with probability $\mathbb{P}_{\mathcal{D}}(\mathcal{\mathcal{E} }) \geqslant 1-p$, the suboptimality of Algorithm \ref{ALGO:PEVI-UCB_General} satisfies
      \#\label{eq:abso_subopt_general}
        %V_1^{\pi,\widehat{v}}(x)-V_1^{\widehat{\pi},v}(x) \leqslant         
        &\abso{V_1^*(x)-V_1^{\pihat,\nuhat}(x)} \notag\\
       \leqslant & 2\max\{\sup\limits_{\nu}\sum_{h=1}^H\expect_{\pi^*,\nu}\left[\Gamma_h\stateph|s_1=x\right], \\
        &\qquad\qquad \sup\limits_{\pi}\sum_{h=1}^H\expect_{\pi,\nu^*}\left[\Gamma_h\stateph|s_1=x\right]\},    \notag    
        %\sum_{h+1}^H(\mathbb{E}_{\pi,\widehat{v}}\left[\iota^{(1)}_{h}(s_h,a_h,b_h)|s_1 = x]-\mathbb{E}_{\widehat{\pi},v}[\iota^{(2)}_{h}(s_h,a_h,b_h)|s_1 = x])\begin{theorem}[Suboptimality of Algorithm \ref{ALGO:PEVI-UCB_General}]\label{theroem:abso_subopt
      \#
      where expectation $\expect_{\pi^*,\nu}$ is taken respect to the trajectory induced by $(\pi^*,\nu)$ in the underlying MG and $\expect_{\pi^*,\nu},\expect_{\pi,\nu^*}$ are taken with respect to $\mbp_\mcd$ (\weir{typo here})
    \end{theorem}
    \begin{proof}[Proof of Theorem \ref{theorem:general_gap_upperb}]
      See \S  B.1 for detailed proof.
    \end{proof}

\subsection{Application to Linear Markov Game}\label{se:LMG}
 % \subsubsection{Linear Asumption and Basic Property of Linear Game}
    Now, We introduce the notion of Linear Markov Game. 
    \begin{assumption} \label{asump:linear_game}
        A linear Markov Game is a Markov Game with a known state function $\phi: \mathcal{S}\times \mathcal{A}_1 \times \mathcal{A}_2 \rightarrow \mathbb{R}^{d}$ , $d$ unknown (signed) measures $\mu_h = (\mu_h^{(1)},\mu_h^{(2)},\cdots,\mu_h^{(d)})$ over state space $\mathcal{S}$ and unknown vectors $\theta_h\in \mathbb{R}^{d}$ such that the expectation of the reward function and the transition kernel have the following form.
         \begin{align}\label{def:linear_eprw}
          &\expect \left[r_h(s,a,b)\right] = \phi\statep^\T\theta_h \\
          & \mathbb{P}_h(x|s_h =s, a_h = a, b_h=b) = \phi\statep^\T\mu_h(x)
         \end{align}
         for all $(s,a,b) \in \mathcal{S}\times\mathcal{A}_1 \times \mathcal{A}_2$. Besides, we assume that  \[ \Vert\phi(s,a,b)\Vert \leqslant 1 ,\quad r_h\statep \in [-1,1],\quad \normof{\theta_h}\leqslant \sqrt{d}, \quad  \int_{x \in \mathcal{S}}\normof{\mu_h(x)}\text{d}x \leqslant \sqrt{d}\]
         for all  $\statep \in \mathcal{S}\times\mathcal{A}_1 \times \mathcal{A}_2, h\in [H] $ 
        \end{assumption}
      $\quad$First, we note that by the definition of the Bellman operator and under Assumption \ref{asump:linear_game}, the Bellman operator $(\bellman\valuefunhat)(s,a,b) $ is linear.
        \begin{align} \label{eq:linear_of_bellman}
         (\bellman\valuefunhat)(s,a,b) &= \expect\left[r(s,a,b)+\valuefunhat(s_{h+1}) |s_h=s,a_h=a, b_h=b\right] \notag  \\
         &= \phi\statep^\T(\theta_h+\int_{x \in \mathcal{S}}\valuefunhat(x)\mu_h (x)\text{d}x) = \phi\statep^\T\omega
        \end{align}
        The last equity holds if we let 
        $\omega = \theta_h+\int_{x \in \mathcal{S}}\valuefunhat(x)\mu_h(x)\text{d}x $. As a result of linearity, we can construct the estimated Bellman operator to be $\bellmanhat\valuefunhat_{h+1}^{(i)}(s,a,b) = \phi(s,a,b)^\T\widehat{\omega}_h^{(i)}$. We use least squares approximation here i.e., we select $\widehat{\omega}_h^{(i)} = \mathop{\text{argmin}}\limits_{\omega \in \mathbb{R}^d} \left(\lambda\normof{\omega}^2+M_h(\omega)\right)$, where the empirical mean squared Bellman error $M_h(\omega)$ is defined to be 
        \[M_h(\omega) = \sum_{\tau=1}^K\left(r_h^\tau+\valuefunhat_{h+1}^{(i)}(x_{h+1}^\tau)-\phi\statepht^\T\omega\right)^2\]
         $\widehat{\omega}_h^{(i)}$ has closed form $\Lambda_h^{-1}\sum_{\tau = 1}^K\left(r_h^{\tau} + \valuefunhat^{(i)}_{h+1}(s_{h+1}^{\tau})\right) $, which give us the Algorithm \ref{ALGO:PEVI-UCB_linear}.

%  \subsubsection{Algorithm and Main Result}
  \begin{algorithm}[h] 
    \caption{PEVI-UCB for Linear Markov Game}
    \begin{algorithmic}[1]
    \STATE Input Dataset $\mathcal{D} = \{(s_h^{\tau},a_h^{\tau},b_h^{\tau},r_h^{\tau})\}_{h=1,\tau = 1}^{H,K}$
    \STATE Initialize $\valuefunhat^{(1)}_{H+1},\valuefunhat^{(2)}_{H+1}$ as zero functions.
    \STATE \textbf{For} step $h = H ,H-1, \ldots ,1$ \textbf{do:}
    \STATE \hspace{0.15in} Construct $(\bellmanhat\valuefunhat_{h+1}^{(i)})(\cdot,\cdot,\cdot),\Gamma_h(\cdot,\cdot,\cdot)$ based on the data .
    \STATE  \hspace{0.15in} Set $\Lambda_h \leftarrow \lambda I + \sum_{\tau = 1}^K \phi\statepht^\T \phi\statepht$
    \STATE  \hspace{0.15in}  Set $\widehat{\omega}^{(1)}_h \leftarrow \Lambda_h^{-1}\sum_{\tau = 1}^K\left(r_h^{\tau} + \valuefunhat^{(1)}_{h+1}(s_{h+1}^{\tau})\right)$
    \STATE  \hspace{0.15in}  Set $\widehat{\omega}^{(2)}_h \leftarrow \Lambda_h^{-1}\sum_{\tau = 1}^K\left(r_h^{\tau} + \valuefunhat^{(2)}_{h+1}(s_{h+1}^{\tau})\right)$
    \STATE  \hspace{0.15in}  Set $\qfunhat^{(1)}_h(\cdot,\cdot,\cdot) \leftarrow \mathrm{\Pi}_h\left(\phi(\cdot,\cdot,\cdot)^\T\widehat{\omega}^{(1)}_h - \beta\sqrt{\phi(\cdot,\cdot,\cdot)^T\Lambda_h^{-1}\phi(\cdot,\cdot,\cdot)}\right)$
    \STATE  \hspace{0.15in}  Set  $\qfunhat^{(2)}_h(\cdot,\cdot,\cdot) \leftarrow \mathrm{\Pi}_h\left(\phi(\cdot,\cdot,\cdot)^\T\widehat{\omega}^{(2)}_h + \beta\sqrt{\phi(\cdot,\cdot,\cdot)^T\Lambda_h^{-1}\phi(\cdot,\cdot,\cdot)}\right)$
    \STATE  \hspace{0.15in} Set $(\pihat_h,\vhat_h) \leftarrow \text{FIND\_NE} \left(\qfunhat_h^{(1)}(\cdot,\cdot,\cdot),\qfunhat_h^{(2)}(\cdot,\cdot,\cdot) \right)$
    \STATE  \hspace{0.15in} Set $\valuefunhat^{(1)}_h(s) \leftarrow \langle\qfunhat_h^{(1)}(s,\cdot,\cdot),\pihat_h(\cdot|s)\otimes \vhat_h(\cdot|s)\rangle_{\mathcal{A}_1 \times \mathcal{A}_2 }$
    \STATE  \hspace{0.15in} Set $\valuefunhat^{(2)}_h(s) \leftarrow \langle\qfunhat_h^{(2)}(s,\cdot,\cdot),\pihat_h(\cdot|s)\otimes \vhat_h(\cdot|s)\rangle_{\mathcal{A}_1 \times \mathcal{A}_2 }$
    \STATE  \textbf{End for}
    \STATE   Output Pess\_Linear$(\mathcal{D}) = \{(\pihat_h,\vhat_h)\}_{h=1}^H$.

    \end{algorithmic}\label{ALGO:PEVI-UCB_linear}
  \end{algorithm}
    Now we consider a class of function 
    \[\mathcal{Q}^{(i)}:=\{\mathrm{\Pi}_h\left(\phi\statep^\T\omega+(-1)^i\beta\sqrt{\phi\statep^\T A\phi\statep} \right): \normof{\omega}\leqslant H\sqrt{\dfrac{Kd}{\lambda}},\normof{A}\leqslant \sqrt{d} \} \label{def:qclass}\]
    By Lemma \ref{lemma:est_of_omega}, $\qfunhat^{(i)}_h \in \mathcal{Q}^{(i)}$. Let $\mathcal{Q}^{(i)}_\epsilon$ be the $\epsilon$- covering of $\mathcal{Q}^{(i)}$ with respect to $\ell_{\infty} $ norm. We present subroutine FIND\_NE Algorithm in Algorithm \ref{ALGO:PEVI-UCB_linear}.
    \han{I think we should use FIND\_CCE. It seems that CCE is enough for our proof.}
  \begin{algorithm}[h] 
    \caption{FIND\_NE}
    \begin{algorithmic}[1]
      \STATE \textbf{Input} $\left(\qfunhat_h^{(1)}(\cdot,\cdot,\cdot),\qfunhat_h^{(2)}(\cdot,\cdot,\cdot) \right)$ and parameter $\epsilon > 0$
      \STATE Choose a pair  $\left(\overline{Q}_h^{(1)}(\cdot,\cdot,\cdot),\overline{Q}_h^{(2)}(\cdot,\cdot,\cdot) \right)$ from $\mathcal{Q}_{\epsilon}^{(1)} \times \mathcal{Q}_{\epsilon}^{(2)}$ satisfying 
          \[\normof{\qfunhat_h^{(1)}-\overline{Q}_h^{(1)}}_{\infty} \leqslant \epsilon, \normof{\qfunhat_h^{(2)}-\overline{Q}_h^{(2)}}_{\infty} \leqslant \epsilon\]  
      \STATE  For input $x$ ,let $(\pihat_h,\vhat_h)$ be the NE of the matrix game with payoff matrix
        \[\overline{Q}_h^{(1)}(x,\cdot,\cdot)\  \text{for P1} \quad \text{and} \quad \overline{Q}_h^{(2)}(x,\cdot,\cdot)\  \text{for P2}\]
      \STATE \textbf{Output:} \text{FIND\_NE}$\left(\qfunhat_h^{(1)}(\cdot,\cdot,\cdot),\qfunhat_h^{(2)}(\cdot,\cdot,\cdot) \right) = (\pihat_h,\vhat_h)$
    \end{algorithmic}\label{Algo:CCE}
  \end{algorithm}

      $\quad$ We use Algorithm \ref{Algo:CCE}  here rather than directly find the NE of $\qfunhat_h^{(i)}$ for some technical reasons. Since the value function and $\phi\statepht$ both depend on the past data, the usual approach to the analysis of such an algorithm is concentration. However, as \citep{xie2020learning} shows that an $\epsilon$-cover of the $Q$-function does not imply an $\epsilon$-covering of the NE value. In order to analyse the algorithm, we use Algorithm \ref{Algo:CCE} to avoid this situation. Moreover, \citep[Appendix D]{xie2020learning} proposes an efficient way to calculate the $\epsilon-$ approximated Q-function in FIND\_NE(Algorithm \ref{Algo:CCE}). It is still an open problem whether this complication is necessary. 

      $\quad $Choosing proper parameter, we are able to prove that the $\Gamma_h(\cdot,\cdot,\cdot) = \beta\sqrt{\phi(\cdot,\cdot,\cdot)^\T\Lambda_h^{-1}\phi(\cdot,\cdot,\cdot)}$ is a $p$-uncertainty quantifier.\\
      \begin{lemma} \label{lemma_uncerty_linear}
        In Algorithm \ref{ALGO:PEVI-UCB_linear}, we set
        \[\lambda = 1 ,\quad\epsilon = \dfrac{dH}{K}, \quad \beta = cdH\sqrt{\zeta} , \text{where}\quad   \zeta = \log(\frac{2dKH}{p})  \]
        Here $c$ is an absolute constant and $p \in (0,1)$ is the confidence parameter. Then, with probability $1-p$, we have
        \#  
        &|\bellmanhat \widehat{V}_{h+1}^{(i)}(s,a,b)-\phi(s,a,b)^\T \widehat{\omega}_h^{(i)}| \notag\\
        &\qquad \leqslant  \beta\sqrt{\phi\statep^\T\Lambda_h^{-1}\phi\statep} \label{ineq:uncerty_linear}
        \#
         holds  for all $ (s,a,b) \in \mathcal{S} \times \mathcal{A}_1 \times \mathcal{A}_2,h\in [H],i = 1,2.$ 
      \end{lemma}
      \begin{proof}[Proof of Lemma \ref{lemma_uncerty_linear}]
        See Appendix B.2 for detailed proof.
      \end{proof} 

      We introduce the notion of Related Uncertainty to characterize the suboptimality of Algorithm \ref{alg1}. 

      \begin{definition}
        Given an MG $\mcm$ and a dataset $\mcd$ that is compliant with $\mcm$, for an optimal policy pair $(\pi^*,\nu^*)$, the Related Uncertainty of $(\pi^*,\nu^*)$ with respect to $\mcd$ is defined as
        \begin{equation}
        \begin{aligned} \label{def:related_info}
         &\ri(\mcd, \pi^*, \nu^*,x) \notag\\
         &\qquad= \max \Big\{\sup\limits_{\nu}\sum_{h=1}^H\expect_{\pi^*,\nu}\left[\sqrt{\phi_h^\T\Lambda_h^{-1}\phi_h}|s_1=x\right], \notag\\
         & \qquad\qquad \sup\limits_{\pi}\sum_{h=1}^H\expect_{\pi,\nu^*}\left[\sqrt{\phi_h^\T\Lambda_h^{-1}\phi_h}|s_1=x\right]\Big\} \notag 
        \end{aligned}
        \end{equation}
        where $x$ is the initial state and expectation $\expect_{\pi^*,\nu}$ is taken respect to randomness of the trajectory induced by $(\pi^*,\nu)$ in the underlying MG given the fixed matrix $\Lambda_h$.  
        
        We also define the Related Uncertainty with respect to the dataset $\cD$ as 
        \begin{equation}
        \ri(\mcd,x) = \inf\limits_{(\pi^*,\nu^*)  \text{optimal policy}}\ri(\mcd, \pi^*, \nu^*,x)
        \end{equation}
      \end{definition}
    \weir{We may first provide the theoretical result and then illustrate the concept of RU. This allows us to directly relate RU to the suboptimality.} \han{yes, i will write the main result in sec 3}
    Therefore, we can reformulate Theorem~{xxxxx} as:
    \begin{equation}
        \label{eqn:rewrite_theorem2}
        \sub((\hat{\pi}, \hat{\nu}), x) \leq XXX\ri(\cD, x).
    \end{equation}
    To illustrate the concept of Related Uncertainty, we consider the following matrix game with $H = 1$, $\cS=\{x\}$, and the payoff matrix:
        \begin{equation*}
          Q = \left(
          \begin{array}{ccc}
            0.5 & \mathbf{-1} & 0  \\
            \mathbf{1} & \textcolor{red}{0} & \mathbf{1}  \\
            0 & \mathbf{-1} & 0  \\
          \end{array}\right).
          %\caption{Illustration of the concept of Related Uncertainty:}
        \end{equation*}
        Element $Q_{ij}$ is the expected reward if the max-player takes action $i$ and the min-player takes action $j$. The NE of this game is action pair $(a_2,b_2)$. The set of action pairs induced by $\sup_\nu \Eb_{\pi^*,\nu}$ and $\sup_\pi \Eb_{\pi, \nu^*}$ is $\{(a_1,b_2),(a_2,b_2),(a_2,b_1),(a_2,b_3),(a_3,b_2)\}$. With $\phi(s, a_i, b_j) = (e_{2(i-1)+j})$ where $e_k$ is the $k$-th orthonormal basis of $\RR^{9}$. We define $n_{ij}$ as the times that $(a_i, b_j)$ is taken in $\cD$. Then, we have
        $$
        \begin{aligned}
        \sup_\nu \expect_{\pi^*,\nu}\left[\sqrt{\phi_h^\T\Lambda_h^{-1}\phi_h}|s_1=x\right] &= (\lambda + \min_j n_{2, j})^{-1/2},\\
        \sup_\pi \expect_{\pi,\nu^*}\left[\sqrt{\phi_h^\T\Lambda_h^{-1}\phi_h}|s_1=x\right] &= (\lambda + \min_in_{i,2})^{-1/2},
        \end{aligned}
        $$
        which implies that 
        $$\ri(\cD,x) = \ri(\mcd, \pi^*, \nu^*,x) = (\lambda + n^*)^{-1/2},$$
        where $n^* = \min\{\min_j n_{2,j}, \min_i n_{i,2}\}$. Therefore $\ri(\cD,x)$ measures how well the dataset $\mcd$ covers the action pairs induced by $(\pi^*,\nu)$ and $(\pi, \nu^*)$ where $\pi$ and $\nu$ are arbitrary. Notably, the action pair that does not lie in the set will not influence $\ri(\cD,x)$. 

        We remark that in the MARL case, one cannot expect to learn a good policy under the assumption that $\cD$ covers the NE $(\pi^*, nu^*)$ well as in the single-agent RL case \cite{jin2020pessimism}. Instead, the instance above illustrates that if $\cD$ covers $(\pi, \nu^*)$ and $(\pi^*, \nu)$ for all policies $\pi$ and $\nu$ well, NE policy learning is possible. This is indeed the case as we have the following information-theoretic lower bound.
        
        
        \quad We remark that in the offline situation, finding the NE value function of a MG can be rather difficult due to insufficient coverage of the dataset. In the MDP case \citep{cai2020provably}, after pessimism process, all the Q-function of actions are underestimated. If the dataset covers the optimal policy sufficiently well, the estimated Q-function of the optimal action will be  greater than all other actions' Q-function regardless of whether other actions are covered well enough or not. \weir{Because}
        $$\hat{Q}(s, a^*) \geq Q* - \epsilon > \hat{Q}(s,a) > Q(s,a).$$
        This follows from the fact that if they are covered well, their estimated Q-function will approximate the real Q-function pretty well, whose value are less than the optimal Q-function. If they are not covered well enough, their Q-function will be far less than the optimal Q-function because of pessimism process.
        
        \quad However, in the case of MG, the situation become worse since our goal is not to maximize the reward but to find a approximated value function of NE. The NE value can be easily influenced due to lack of information after the pessimism process. For instance, in an extreme case of game mentioned above, if the dataset only covers the action of the optimal actions pair, the payoff matrix of players in Algorithm \ref{ALGO:PEVI-UCB_linear} may become   
        \begin{equation*}
          \left(
          \begin{array}{ccc}
            (-1,1) & (-1,1) & (-1,1)  \\
            (-1,1) & (0,0) & (-1,1) \\
            (-1,1) & (-1,1) & (-1,1)  \\
          \end{array}\right)
        \end{equation*}    
          The entries of the matrix are $(\qfunhat^{(1)}_1(a_i,b_j),\qfunhat^{(2)}_1(a_i,b_j))$. As we can see from the matrix, action pairs $(a_i,b_j),(a_2,b_2),i,h \neq 2 $ are NE of the general-sum game. The pessimism process create a great many 'spurious NE'. The example tells us that in MG, we need more information about the game to determine the value function.  The situation become much more complicated and worse when some action pairs are covered while others are not.
          
          \quad An important observation about Zero-Sum two-player MG allows us to use less information to do so, which may no longer hold in MG with three agents or more. The related information of the optimal actions can help us eliminate spurious NE. We illustrate this point via a special case. We consider a MG with $H = 1$. The payoff matrix is $(r_{ij})_{1 \leqslant i,j \leqslant n}$. Supposed that $(a_1,b_1)$ is the NE. If actions $(a_1,b_i),(a_j,b_1),1 \leqslant i,j \leqslant n$ are covered sufficiently well, we can regard that 
          \$
          &\qfunhat^{(1)}_1(a_1,b_j) \approx  \qfunhat^{(2)}_1(a_1,b_j) \approx r_{1j} \\ %\text{ and }\quad 
          &\qfunhat^{(1)}_1(a_i,b_1) \approx  \qfunhat^{(2)}_1(a_i,b_1) \approx r_{i1} 
          \$
           And depend on the dataset 
           $$\qfunhat^{(1)}_1(a_i,b_j) =  r_{ij} - \delta_{ij},\quad  \qfunhat^{(2)}_1(a_i,b_j) =r_{ij} + \delta_{ij},\quad i \neq 1, j\neq 1 , \delta_{ij} >0$$
          If the action pair $(a_i,b_j)$  wants to ‘pretend’ to be a NE, it needs to satisfy
          \[r_{ij} - \delta_{ij}\geqslant r_{1j}  \quad \text{and} \quad r_{ij} + \delta_{ij}\leqslant r_{i1} \]
          But because of the property of NE 
          $$r_{11}\geqslant r_{i1} \geqslant r_{ij} + \delta_{ij} ,\quad  r_{11}\leqslant r_{1j} \leqslant r_{ij} - \delta_{ij}$$
          which implies that $\qfunhat^{(k)}_1(a_i,b_j) \approx r_{ij} \approx r_{11} , k = 1,2$. In analogy to this example, we have the following theorem .

      \begin{theorem} \label{theroem:abso_subopt_linear}
        In Algorithm \ref{ALGO:PEVI-UCB_linear}, for any $p \in (0,1)$, under the setting in Lemma \ref{lemma_uncerty_linear}, we have 
        \begin{align}\label{eq:abso_subopt_linear}
          \abso{V_1^*(x)-V_1^{\pihat,\nuhat}(x)} \leqslant 2\beta \ri(\mcd,x) + \dfrac{2dH^2}{K}
        \end{align}

        with probability $1-p$ for any policy pair $(\pi,\nu)$. The expectation is taken with respect to $\mathbb{P}_{\mcd}$.
      \end{theorem}
      \begin{proof}[Proof of Theorem \ref{theroem:abso_subopt_linear}]
        See Appendix B.3 for detailed proof.
      \end{proof}
      \quad Analogy to the good property of Pessimistic Value Iteration in MDP \citep{jin2020provably}, we highlight the following aspect of Theorem \ref{theroem:abso_subopt_linear}.

      \textbf{"Assumption Free" Guarantee:} Theorem \ref{theroem:abso_subopt_linear} only relies on the compliant of dataset $\mcd$ rather than 'uniform coverage' of $\mcd$, which usually fails to hold in practice. Besides, we do not require the affinity between Pess($\mcd$) and the behavior policy $\overline{\pi}$ that induces $\mcd$.
 
      \textbf{Oracle Property:} Because of the pessimistic process, the trajectory of optimal policy 'stands out' when Pess($\mcd$) determine its policy in each step. In other word,  Pess($\mcd$) will autonomously 'support' the  trajectory of optimal policy even though the optimal policy$(\pi^*,\nu^*)$ is unknown a prior.

      \textbf{Outperforming Demonstration:} In practice, apart from the Related Information, the dataset $\mcd$ may not cover a large amount of irrelevant information $(s_h,a_h,b_h)$, which may not cause suboptimality for some algorithm. However, for Pess($\mcd$), the suboptimality of the algorithm only relies on the coverage of Related Information. When Related Information is covered sufficiently well, that is , when $\ri(\mcd,x)$ is sufficiently small, the suboptimality will be relatively small and will not be influenced by the irrelevant information.

      \begin{corollary}[Sufficent Coverage of Related Information]\label{cor:suff}
        Supposed that event
          \begin{equation}\label{event:suff}
            \mathcal{E}_1 = \{\Lambda_h\geqslant I + c_1 \cdot K \cdot \max\{\sup\limits_{\nu}\expect_{\pi^*,\nu}[\phi_h\phi_h^\T|s_1=x],\sup\limits_{\pi}\expect_{\pi,\nu^*}[\phi_h\phi_h^\T|s_1=x] \}\}
          \end{equation}
        happens with probability $1-\xi/2$, setting 
          \[\lambda = 1 \quad \epsilon = \dfrac{dH}{K} \quad \beta = cdH\sqrt{\zeta} \quad \zeta = \log(\dfrac{4dKH}{\xi})\]
        in Algorithm \ref{ALGO:PEVI-UCB_linear}, where the constant $c$ is specified in Lemma \ref{lemma_uncerty_linear}. With probability $1-\xi$, we have 
          \#\text{SubOpt}(\text{Pess}(\mcd),x)\leqslant c''d^{3/2}H^2K^{-1/2}\sqrt{\zeta} \#
          where $c''$ is an absolute constant that only relies on $c$ and $ c'$.
      \end{corollary}
      \begin{proof}
        See Appendix B.4 for detailed proof.
      \end{proof}
      \begin{corollary}[Sufficent Coverage of the Action-State Space]\label{cor_well_exp}
        Supposed the dataset $\mcd = \{(s_h^\tau,a_h^\tau,b_h^\tau,r_h^\tau)\}_{\tau,h=1}^{K,K}$ is induced by a fixed behavior policy $(\bpc)$ in the underlying MG. Let $\lambda_{\text{min}}(A)$ be the smallest eigenvalue of the matrix $A$. There exists a absolute constant $\underline{c}>0$ such that 
        \[\lambda_{\text{min}}(\Sigma_h) \geqslant \underline{c}\quad \text{where} \quad \Sigma_h = \expect_{\bpc}[\phi_h\phi_h^\T ]\quad \forall h \in [H]\]
        setting 
        \$
        \lambda = 1, \quad \epsilon = \dfrac{dH}{K}, \quad \beta = cdH\sqrt{\zeta}, \quad \zeta = \log(\dfrac{4dKH}{\xi})
        \$
        in Algorithm \ref{ALGO:PEVI-UCB_linear} where the constant $c$ is specified in Lemma~\ref{lemma_uncerty_linear}. If $K > c'\log\left(4dH/\xi\right)$ where $c'$ is a constant that only depend on $\underline{c}$, with probability $1-\xi$, we have 
        \[\text{SubOpt}(\text{Pess}(\mcd);x)\leqslant c''dH^2K^{-1/2}\sqrt{\zeta}\]
        where $c''$ is a constant that only depends on $\underline{c}$ and $c'$.
      \end{corollary}
      \begin{proof}
        See section B.5 for detailed proof.
      \end{proof}

==> section4.tex <==
\section{Information Lower Bound}
In this section, we establish the minimax optimality of Theorem~\ref{theroem:abso_subopt_linear} by the following information-theoretical lower bound.

\begin{theorem}\label{theorem:minimax}
 For any algorithm $\algo(\mathcal{D})$, there exists a linear game $\mathcal{M}$ and a dataset $\cD$ that is compliant with the underlying MG $\mcm$, such that when $K$ is large enough, it holds that 
  \begin{equation}\label{ineq:minimax}
    \expect_{\mathcal{D}}\left[\dfrac{\sub\left(\algo(\mathcal{D});x_{0}\right)}{\ri(\mcd,x_0)}\right] \geqslant C',
  \end{equation}
 where $C'$ is an absolute constant and $x_0$ is the initial state. The expectation is taken with respect to $\mathbb{P}_{\mcd}$ where $\algo(\cD)$ is a policy pair constructed based on the dataset $\cD$.
\end{theorem}
The proof is deferred to Appendix~\ref{sec:proof_lower} due to space limit. We sketch the main ideas here. We will construct a special class of linear Markov Games $\mathfrak{M}$ and design a data collecting process that corresponds to the distribution $\PP_\cD(\cdot)$. Then, for any policy pair $(\pi, \nu)$ constructed from $\cD$, we can find two linear MGs $\cM_1$ and $\cM_2$ such that (i) the distributions of $\cD$ are similar when $\cM_1$ and $\cM_2$ are the underlying MG so it is hard to distinguish them based on $\cD$, and (ii) $(\pi, \nu)$ cannot achieve a designed suboptimality for $\cM_1$ and $\cM_2$ simultaneously so the worse game meets our need. 

==> section5.tex <==
\section{Multi-Agent General-Sum Markov Game (MAMG)}\label{sec:main_MAMG}
\han{just consider the two-player setting. define value functions, NE, learning objective (subopt), highly competitive game. necessary and sufficient condition (proposition in Appendix), main theorem }

    In this section, we generalize our previous results to a special class of MAMG.
    
    First, given the output of an algorithm, we define the suboptimality of two-player general sum game to be
    $$ \sub(\mathcal{D},x) = \max \{V^{*,\hat{\nu},1}_1(x)-V^{\hat{\pi},\hat{\nu},1}_1(x),V^{\hat{\pi},\hat{\nu},2}_1(x)-V^{\hat{\pi},*,2}_1(x)\} $$
    
    \han{$$ \sub(\mathcal{D},x) = \max \{V^{*,1}_1(x)-V^{\hat{\pi},*,1}_1(x),V^{*,\hat{\nu},2}_1(x)-V^{*,2}_1(x)\} $$}
   The algorithm PMVI for MAMG is similar to Algorithm \ref{ALGO:PEVI-UCB_General}, except that we construct an approximated Bellman operator $\bellmanhat^{i}(V)$ for each player. Due to the limit of space, we leave the decomposition and algorithm to the Appendix \ref{sec:MAMG}.

    \quad Now, we introduce a special class of MAMG. It turns out that our algorithm works well with this class of game.
    \begin{definition}[Highly Competitive Game]\label{def:hc_game}
        A MAMG $\mcm$ is highly competitive if there exists a NE $(\pi^*,\nu^*)$ of $\mcm$ such that for any policy $(\pi,\nu)$, 
        \[V_h^{*,1}(x) \leqslant V_h^{\pi^*,\nu,1}(x) \qquad V_h^{*,2}(x) \geqslant V_h^{\pi,\nu^*,2}(x) \quad \forall x \in \mathcal{S}, h\in[H]  \label{eq:hc_game}\]
    \end{definition}
    In other words, in highly competitive MAMG, there exist a much more sophisticated balance among players than the common NE. A small perturbation of policy of one player will lead to the increase of reward of the remaining players. 
    
\iffalse
    We call $\{\Gamma^{(i)}_h\}_{h=1,i}^{H,n}$ a $\xi-$ uncertainty quantifier with respect to approximated Bellman operators  $\{\bellmanhat^{(i)}\}_{i=1}^n$ if the following event happens with at least probability $1-\xi$
    \$
    \mathcal{E}' &=\{|\bellmanhat \widehat{V}_{h+1}^{(i)}(s,a)-\mathbb{B}_h\widehat{V}_{h+1}^{(i)}(s,a)|\leqslant \Gamma_h^{(i)}(s,a),\  \\ &\qquad\qquad \forall (s,a) \in \mathcal{S} \times  \mathcal{A},h\in [H],i = 1,\cdots,n \} \label{eq:p_uncerty_MAMG}
    \$
     The following Theorem characterizes the suboptimality of our Algorithm for highly competitive MAMG. 
     
\fi 

    \begin{theorem}[Suboptimality of Highly Competitive MAMG]\label{thm:subopt_for_MAMG}
    Given a highly competitive MAMG $\mcm$ and $\xi$-uncertainty quantifier $\{\Gamma^{(i)}_h\}_{h=1,i}^{H,n}$, when the event $\mathcal{E}'$ happens, the suboptimality of PMVI for MAMG satisfies
    \$
    \sub(\text{PMVI}(\mcd);x) \leq  3\beta \ri(\mathcal{D},x). 
    \$
    \end{theorem}
    \begin{proof}
        See Appendix \ref{sec:MAMG} for detailed proof.
    \end{proof}
     We are able to give a necessary and sufficient condition for a game to be highly competitive. 
     \begin{proposition}[Necessary and Sufficient Condition for a MAMG to be Highly Competitive]\label{prop:NS_MAGA}
        A two-player MAMG $(\mcm, \mbp,\mathcal{A},(r^1,r^2),\mathcal{S},H)$ is highly competitive if and only if there exists a common NE  for the zero-sum games  $(\mcm_1, \mbp,\mathcal{A},r^1,\mathcal{S},H)$ and $(\mcm_2, \mbp,\mathcal{A},r^2,\mathcal{S},H)$. In both of the zero-sum games, player 1 is the max-player while player 2 is the min-player. 
    \end{proposition}
    \begin{proof}
    See Appendix \ref{sec:MAMG} for detailed proof.
    \end{proof}
    
